Advanced Datapath Synthesis using Graph Isomorphism

This paper presents an advanced DAG-based algorithm for datapath synthesis that targets area minimization using logic-level resource sharing. The problem of identifying common specification logic is formulated using unweighted graph isomorphism problem, in contrast to a weighted graph isomorphism using AIGs. In the context of gate-level datapath circuits, our algorithm solves the un- weighted graph isomorphism problem in linear time. The experiments are conducted within an industrial synthesis flow that includes the complete high-level synthesis, logic synthesis and placement and route procedures. Experimental results show a significant runtime improvements compared to the existing datapath synthesis algorithms.

==> systemc.tex <==
\begin{table}[]
\scriptsize
\centering
\label{tbl:systemC}
\begin{tabular}{|l|}
\hline
\begin{tabular}[c]{@{}l@{}}for (i = 0; i \textless 5; i++)\\ \{\\~~if(x $>$ y \&\& x $<$ 2*y)\\~~~~~ f = f - x; \\~~else\\~~~~~~f = f + y;\\ \}\end{tabular} \\ \hline
\end{tabular}
\caption{C++ implementation example}
\vspace{-3mm}
\end{table}
